Balancing Biases and Preserving Privacy on Balanced Faces in the Wild

There are demographic biases present in current facial recognition (FR) models. To measure these biases across different ethnic and gender subgroups, we introduce our Balanced Faces in the Wild (BFW) dataset. This dataset allows for the characterization of FR performance per subgroup. We found that relying on a single score threshold to differentiate between genuine and imposters sample pairs leads to suboptimal results. Additionally, performance within subgroups often varies significantly from the global average. Therefore, specific error rates only hold for populations that match the validation data. To mitigate imbalanced performances, we propose a novel domain adaptation learning scheme that uses facial features extracted from state-of-the-art neural networks. This scheme boosts the average performance and preserves identity information while removing demographic knowledge. Removing demographic knowledge prevents potential biases from affecting decision-making and protects privacy by eliminating demographic information. We explore the proposed method and demonstrate that subgroup classifiers can no longer learn from features projected using our domain adaptation scheme. For access to the source code and data, please visit https://github.com/visionjo/facerec-bias-bfw.

==> ita-fig.tex <==

\begin{comment}
\begin{figure}
    \centering
        \begin{tikzpicture}[scale=.6]
              % b* shade
              \path[draw, shade, left color=blue, right color=yellow, opacity=.6] 
                (0,0,0) node[below] {$-b^*$} -- (5,2.0,0) node[below] {$+b^*$}
                -- (5, 2.5, 0) -- (0, 0.5, 0) -- cycle;
            
              % a* shade
              \path[draw, shade, left color=green, right color=red, opacity=.6] 
              (0, 2.0, 0) node[below] {$-a^*$} -- (5, 0, 0) node[below] {$+a^*$} 
              -- (5, .5, 0) -- (0, 2.5, 0) -- cycle;
                
              % L* shade
              \path[draw, shade, top color=white, bottom color=black, opacity=.6] 
                (2.65, -1.85, 0) node[right] {$L^*=0$ (Black)} -- (2.65, 4.45, 0)
                node[right] {$L^*=100$ (White)} -- (2.35, 4.3, 0)  -- (2.35, -2., 0) -- cycle;
            
              % b*-axis
              \draw[<->] (0,0.25,0) -- (5, 2.25, 0);
              % a*-axis
              \draw[<->] (0,2.25,0) -- (5, 0.25, 0);
              % L*-axis
              \draw[<->] (2.5,-1.90,0) -- (2.5,4.35,0);
                %   \draw (2.5,0) ellipse (2.5cm and 2.5cm);
                %   \draw (3,0) arc (0:75:3cm);
        \end{tikzpicture}
    \caption{{\textbf{CIE-Lab color model.} The $L$-axis, $a$-axis, and $b$-axis represent the luminance, redness, and yellowness, respectively. The axes $a$-axis and $b$ are span from positive to negative for the presence and absence, respectively, of their colors.}}
    \label{fig:my_label}
\end{figure}

\begin{figure}[t!]
    \centering
    % \begin{subfigure}[t]{\linewidth}
        \includegraphics[width=.6\linewidth]{pdf/face-segmentations.pdf}
    % \end{subfigure}
    \caption{{\textbf{Segmentation to measure tones of skin regions.}}}
    \label{fig:ita:facesegmentation}
\end{figure}



% \begin{figure}[b!]
%     \centering
%     \glsunset{ita}
%     % \glsunset{ita}
% \glsunset{fst}
% %   \begin{subfigure}[t]{\linewidth}
% %     \centering
% %     \scriptsize
% %     {
% %     % \caption{{\textbf{Skin tone type based on the \gls{ita}.} \Gls{ita} values, in degrees (Eq.~\ref{eq:ita}), are categorized per the condition met, where references (\ie \textbf{Ref.}) are shorthand used in the text body.}}
% %     \begin{tabular}{ccc}
% %     \textbf{Criteria} & \textbf{Category} & \textbf{Ref.} \\\midrule 
% %       \rowcolor{verylight}\textcolor{black}{$\text{\gls{ita}}>55^{\circ}$} & \textcolor{black}{Very Light} & \textcolor{black}{\emph{vlt}} \\
% %       \rowcolor{lightb}\textcolor{black}{$48^{\circ}<\text{\gls{ita}}\leq55^{\circ}$} & \textcolor{black}{Light 2}  &  \textcolor{black}{\emph{lt2}}\\
% %       \rowcolor{lighta}\textcolor{black}{$41^{\circ}<\text{\gls{ita}}\leq48^{\circ}$} & \textcolor{black}{Light 1} & \textcolor{black}{\emph{lt1}} \\
% %       \rowcolor{intermb}\textcolor{black}{$34.5^{\circ}<\text{\gls{ita}}\leq41^{\circ}$} & \textcolor{black}{Intermediate 2} & \textcolor{black}{\emph{int2}} \\
% %       \rowcolor{interma}\textcolor{white}{$28^{\circ}<\text{\gls{ita}}\leq34.5^{\circ}$} & \textcolor{white}{Intermediate 1} & \textcolor{white}{\emph{int1}} \\
% %       \rowcolor{tanb}\textcolor{white}{$19^{\circ}<\text{\gls{ita}}\leq28^{\circ}$} & \textcolor{white}{Tanned 2} &  \textcolor{white}{\emph{tan2}} \\
% %       \rowcolor{tana}\textcolor{white}{$10^{\circ}<\text{\gls{ita}}\leq19^{\circ}$} & \textcolor{white}{Tanned 1} &  \textcolor{white}{\emph{tan1}} \\
% %         \rowcolor{dark}\textcolor{white}{$\text{\gls{ita}}\leq10^{\circ}$} & \textcolor{white}{Dark} & \textcolor{white}{\emph{dark}} \\
% %     \end{tabular}
% %     } \caption{Skin tone type based on the \gls{ita}.}\label{fig:fitztypes}
% %   \end{subfigure}\\
  
%     % \begin{subfigure}[t]{\linewidth}
%         \centering
%         {
%         \includegraphics[width=.9\linewidth]{pdf/rain-cloud-ethnicity.pdf}
%         }
%         % \caption{\gls{ita} values per ethnicity.} %\label{fig:fitz:b}
%     % \end{subfigure}
%     \caption{{\textbf{\gls{ita} values per ethnicity.} The \gls{ita} values (Eq.~\ref{eq:ita}), are lighter with increase in value, while the smallest are the darkest. \gls{ita} per ethnic group matches expectations (red, vertical line) shifts from darkest to lightest: Black, Indian, White, and Asian. ITA values are summarized using scattered, box, and distribution.}}
%     % \caption{{\textbf{\gls{ita} measures for skin tone analysis.} \gls{ita} values, in degrees (Eq.~\ref{eq:ita}), are lighter with increase in value, while the smallest are the darkest. Referring to the look-up table (\ref{fig:fitztypes}), \gls{ita} per ethnic group matches expectations from darkest to lightest: Black, Indian, White, and Asian (\ref{fig:fitz:b}). ITA values are summarized using scattered, box, and distribution, with the vertical line pointing to the mean of each.}
%     % }
%     \label{fig:ita:violin}
%     \glsreset{ita}
%     % \glsreset{ita}
% \glsreset{fst}
% \end{figure}

% \begin{table}[h!b]
% \glsunset{ita}
% \glsunset{fst}
%     \centering
%     {
%     \caption{{\textbf{Skin tone type based on the \gls{ita}.} \Gls{ita} values, in degrees (Eq.~\ref{eq:ita}), are categorized per the condition met, where references (\ie \textbf{Ref.}) are shorthand used in the text body.}}
%     \begin{tabular}{ccc}
%     \textbf{Criteria} & \textbf{Category} & \textbf{Ref.} \\\midrule 
%       \rowcolor{verylight}\textcolor{black}{$\text{\gls{ita}}>55^{\circ}$} & \textcolor{black}{Very Light} & \textcolor{black}{\emph{vlt}} \\
%       \rowcolor{lightb}\textcolor{black}{$48^{\circ}<\text{\gls{ita}}\leq55^{\circ}$} & \textcolor{black}{Light 2}  &  \textcolor{black}{\emph{lt2}}\\
%       \rowcolor{lighta}\textcolor{black}{$41^{\circ}<\text{\gls{ita}}\leq48^{\circ}$} & \textcolor{black}{Light 1} & \textcolor{black}{\emph{lt1}} \\
%       \rowcolor{intermb}\textcolor{black}{$34.5^{\circ}<\text{\gls{ita}}\leq41^{\circ}$} & \textcolor{black}{Intermediate 2} & \textcolor{black}{\emph{int2}} \\
%       \rowcolor{interma}\textcolor{white}{$28^{\circ}<\text{\gls{ita}}\leq34.5^{\circ}$} & \textcolor{white}{Intermediate 1} & \textcolor{white}{\emph{int1}} \\
%       \rowcolor{tanb}\textcolor{white}{$19^{\circ}<\text{\gls{ita}}\leq28^{\circ}$} & \textcolor{white}{Tanned 2} &  \textcolor{white}{\emph{tan2}} \\
%       \rowcolor{tana}\textcolor{white}{$10^{\circ}<\text{\gls{ita}}\leq19^{\circ}$} & \textcolor{white}{Tanned 1} &  \textcolor{white}{\emph{tan1}} \\
%         \rowcolor{dark}\textcolor{white}{$\text{\gls{ita}}\leq10^{\circ}$} & \textcolor{white}{Dark} & \textcolor{white}{\emph{dark}} \\
%     \end{tabular}\label{tab:fitztypes}
%     }
    
% \glsreset{ita}
% \glsreset{fst}
% \end{table}
\end{comment}


\begin{comment}

\begin{figure*}[h!b]
\centering
         \includegraphics[width=\linewidth]{pdf/page-1-teaser-barplot.pdf}
\caption{\textbf{Percent difference from intended FPR.} \emph{Left:} $t_g$ yields an FPR that spans up to 200\% the intended (\ie WM for 1e-4); the F subgroups perform worse than intended for all, while M's overshoot the intended performances besides IM at FPR=1e-4. \emph{Right:} \emph{Subgroup-specific thresholds} $t_o$ reduces the difference closer to zero. Furthermore, the proposed method, which does not assume knowledge of attribute information at inference like for $t_o,$ mitigates the inconsistencies in the \emph{global FPR} versus \emph{subgroup-specific FPR} (\ie \emph{middle}). Similar to the results in Table~\ref{tab:ethnicy-far}, the variations nearly reduce by a 1/2. So, although there are small differences, the percent difference for different subgroups is much fairer for features adapted to our approach.}
\label{fig:page1-teaser-barplot}
\end{figure*}
\end{comment}
